Qubit-Boson Hybrid Beam-Splitter Gate with Kerr Nonlinearity in Circuit QED for Many-Body Dynamics

We introduce a hybrid qubit-boson beam-splitter gate in which a microwave cavity mode couples to an exchange-dressed two-level subsystem of an interacting two-qubit system in the presence of Kerr nonlinearity. Starting from a general circuit quantum electrodynamics (cQED) model, we derive the corresponding hybrid qubit-cavity interaction, develop its open-system description including photon- and qubit-sector-bath-induced dissipation and obtain in the weak-dissipation regime an analytical expression for the average gate fidelity. We further identify carbon-nanotube circuit QED as a concrete platform for implementing and controlling the gate, provide a representative operating regime and perform noiseless and noisy numerical simulations to study the gate dynamics and benchmark the analytical results. Beyond this implementation route, the proposed hybrid primitive provides a natural building block for many-body dynamics, including quantum-cellular-automaton (QCA) and lattice-gauge-inspired architectures and, through its collision-model reformulation, also suggests connections to noisy QCA, non-Markovian extensions and reservoir-style quantum information processing.

==> main/main_Lindblad.tex <==
% =========================
\section{Open-system dynamics and Lindblad description}
\label{sec:lindblad_main}
% =========================
\begin{comment}    
\textcolor{red}{We model Markovian dissipation due to (i) a photon bath coupled to the cavity quadrature, which the weak-Kerr regime (bath cannot resolve Kerr-split transitions), the cavity dissipator is
well-approximated by the usual collapse operator $a$ and (ii) a phonon bath coupled}
\end{comment}

% --- Lindblad: Hamiltonians and setup ---
\subsection{System--bath Hamiltonians}

We model dissipation by coupling the qubits+cavity system to (i) a photon bath and (ii) a phonon bath. 
The total Hamiltonian is
\begin{equation}
H_{\mathrm{tot}}=H_S+H_\gamma+H_{\gamma S}+H_\nu+H_{\nu S},
\end{equation}
with the system Hamiltonian of Eq. ~\eqref{eq:H_full_main}.
The photon bath and coupling are
\begin{align}
H_\gamma&=\sum_k \omega_k b_k^\dagger b_k,\\
H_{\gamma S}&=S_{\gamma} \otimes B_\gamma,\qquad 
B_\gamma=\sum_k (f_k b_k^\dagger+f_k^\ast b_k),\\
& S_{\gamma}=(a+a^\dagger), \\
\end{align}
and the phonon bath and coupling are
\begin{align}
H_\nu&=\sum_q \omega_q c_q^\dagger c_q,\\
H_{\nu S}&=S_\nu\otimes B_\nu,\qquad 
B_\nu=\sum_q (h_q c_q^\dagger+h_q^\ast c_q),\\
S_\nu&=\sum_{i=1}^2\left(\alpha_i\sigma_x^{(i)}+\beta_i\sigma_z^{(i)}\right).
\label{eq:Snu_def_main}
\end{align}
%
where $\alpha_i$ describes transverse (flip) coupling
and $\beta_i$ longitudinal (dephasing-type) coupling.
% 
\subsection{Lindblad derivation}
The master equation is derived using the standard Born--Markov and secular
(Davies) procedure. In this approach the system operators coupled to the baths
are decomposed into eigenoperators of the system Hamiltonian,
\begin{equation}
S(\omega)=\sum_{\epsilon-\epsilon'=\omega}
\Pi(\epsilon)\,S\,\Pi(\epsilon'),
\qquad
[H_S',S(\omega)]=-\omega S(\omega),
\end{equation}
where $\Pi(\epsilon)$ projects onto the eigenspace of the system Hamiltonian
with energy $\epsilon$.
Within this framework the reduced density matrix obeys a Lindblad master equation
\begin{equation}
\begin{split}
&\dot{\rho}
=
-i[H(t),\rho]
+
\sum_{\omega}
\mathcal{D}[L(\omega)]\rho, \\
&\mathcal{D}[L]\rho
=
L\rho L^\dagger
-
\frac12\{L^\dagger L,\rho\},
\label{eq:lindblad_main_revised}
\end{split}
\end{equation}
where the jump operators are
\begin{equation}
L(\omega)=\sqrt{\gamma(\omega)}\,S(\omega),
\end{equation}
and $\gamma(\omega)$ denotes the bath spectral rate evaluated at frequency
$\omega$.

We proceed as in Sec.~\eqref{sec:red_sideband_ham}, simplifying the system Hamiltonian via a polaron transformation—treating the cavity within the weak-Kerr approximation—which removes the longitudinal qubit--cavity coupling. We then diagonalize the parallel and antiparallel sectors (see Supplemental Material). For the Lindblad derivation, however, we do not move to the interaction picture, as this would complicate the construction of the dissipators.

Throughout the derivation we retain the polaron-induced exchange term $H_J$ in the coherent system Hamiltonian, since it provides the cavity-assisted interaction responsible for the gate dynamics. However, when constructing the photon and phonon dissipators we perform the eigenoperator decomposition with respect to a reference Hamiltonian $H_0$ rather than the full Hamiltonian.

This approximation is valid provided that the additional splittings induced by $H_J$ remain unresolved by the baths, i.e.\ when the hybridization scale $g_J\sqrt{n_{\max}+1}$ is small compared to the relevant bath linewidths (e.g.\ $\kappa$). In this regime the baths effectively probe the unhybridized spectrum, while $H_J$ still contributes coherently to the system dynamics.

%
\subsection{Photon-induced channels}
%
After the polaron transformation, in the weak-Kerr regime, where the bath cannot resolve Kerr-split transitions 
(i.e.\ $2|\chi|n_{\max}\ll \kappa$) the photon coupling writes

\begin{equation}
S_{\gamma}^{P}=(a+a^\dagger-2 \lambda Z) .
\end{equation}

The cavity dissipation is well approximated by the standard collapse operators
\begin{equation}
L_a=\sqrt{\kappa_\downarrow}\,a,
\qquad
L_{a^\dagger}=\sqrt{\kappa_\uparrow}\,a^\dagger.
\label{eq:cavity_jumps}
\end{equation}

Here $\kappa_\downarrow=\gamma_\gamma(\omega_c)$ and 
$\kappa_\uparrow=\gamma_\gamma(-\omega_c)$ are the photon emission and absorption rates 
set by the bath spectral density at $\pm\omega_c$. 
%


Because of the longitudinal qubit--cavity coupling, 
the polaron transformation generates an additional qubit operator component 
proportional to $Z=\sigma_z^{(1)}-\sigma_z^{(2)}$. 
Projecting onto the dressed eigenbasis of the two-qubit Hamiltonian 
(see Supplemental Material), one obtains effective photon-induced 
transitions in the antiparallel manifold 
$\{|AP+\rangle,|AP-\rangle\}$ with splitting 
$\omega_{\mathrm{ap}}=2\Omega_{\mathrm{ap}}$.

The corresponding collapse operators are

\begin{equation}
\begin{split}
L_{\gamma,+}
&=
\sqrt{\gamma_\gamma(\omega_{\mathrm{ap}})}\,
(4\lambda\sin 2\theta_{\mathrm{ap}})\,
|AP-\rangle\langle AP+|,
\\
L_{\gamma,-}
&=
\sqrt{\gamma_\gamma(-\omega_{\mathrm{ap}})}\,
(4\lambda\sin 2\theta_{\mathrm{ap}})\,
|AP+\rangle\langle AP-|,
\\
L_{\gamma,0}
&=
\sqrt{\gamma_\gamma(0)}\,
(4\lambda\cos 2\theta_{\mathrm{ap}})
\big(|AP+\rangle\langle AP+|\\
&-|AP-\rangle\langle AP-|\big).
\label{eq:photon_qubit_jumps}
\end{split}
\end{equation}

The first two operators describe photon-induced relaxation and excitation 
between the dressed antiparallel states, 
while $L_{\gamma,0}$ generates pure dephasing in that manifold. Notably, the parallel manifold $\{|P\pm\rangle\}$ is unaffected by photon-induced qubit jumps 
because $Z$ annihilates $|00\rangle$ and $|11\rangle$.
\subsection{Phonon-induced channels}
%
Within the polaron frame, the phonon
coupling operator writes
%
\begin{equation}
S_\nu^{P}
=
S_\nu^{(0)}+S_\nu^{(1)}+\mathcal O(\lambda^2),
\label{S:eq:Snu_split}
\end{equation}
with
\begin{align}
S_\nu^{(0)}
&=
\sum_{i=1}^2\big(\alpha_i\sigma_x^{(i)}+\beta_i\sigma_z^{(i)}\big),
\label{S:eq:Snu0_def}
\\
S_\nu^{(1)}
&=
2i\lambda(a^\dagger-a)
\big(\alpha_1\sigma_y^{(1)}-\alpha_2\sigma_y^{(2)}\big).
\label{S:eq:Snu1_def}
\end{align}
%
\textcolor{red}{In the main derivation below we construct
the phonon dissipator from $S_\nu^{(0)}$ only, thus neglecting $S_\nu^{(1)}$.}
Decomposing $S_\nu$ in the dressed eigenbasis produces three classes of transitions:


\paragraph{Parallel manifold $\mathcal H_{\rm p}$.}
%
\begin{equation}
\begin{split}
L_{\nu,{\rm p}}(\pm\omega_{\rm p})
&=
-\sqrt{\gamma_\nu(\pm\omega_{\rm p})}(\beta_1+\beta_2)\sin{(2\theta_{\rm p})}
\ket{P\mp}\!\bra{P\pm},\\
L_{\nu,{\rm p}}(0)
&=
\sqrt{\gamma_\nu(0)}(\beta_1+\beta_2)\cos{(2\theta_{\rm p})}
\Big(\ket{P+}\!\bra{P+}\\
&-\ket{P-}\!\bra{P-}\Big)\ ,
\end{split}
\end{equation}

\paragraph{Antiparallel manifold $\mathcal H_{\rm ap}$.}
%
\begin{equation}
\begin{split}
L_{\nu,{\rm ap}}(\pm\omega_{\rm ap})
&=
-\sqrt{\gamma_\nu(\pm\omega_{\rm ap})} (\beta_1-\beta_2)\sin{(2\theta_{\rm ap})}\\
&\ket{\mathrm{AP}\mp}\!\bra{\mathrm{AP}\pm},\\
L_{\nu,{\rm ap}}(0)
&=
\sqrt{\gamma_\nu(0)}\,(\beta_1-\beta_2)\cos{(2\theta_{\rm ap})}\,
\Big(\ket{\mathrm{AP}+}\!\bra{\mathrm{AP}+}\\
&-\ket{\mathrm{AP}-}\!\bra{\mathrm{AP}-}\Big).
\end{split}
\end{equation}

\paragraph{Cross-manifold transitions}
Single-qubit flip terms proportional to $\sigma_x^{(i)}$ 
induce transitions between parallel and antiparallel manifolds:
\begin{equation}
L_{\nu,\mu\mu^{\prime}}
=
\sqrt{\gamma_\nu(\omega_{\mu\mu^{\prime}})}
\,
C_{\mu\mu^{\prime}}
\,
|A\mu\rangle\langle P\mu^{\prime}|, \mu,\mu'\in\{+,-\},
\end{equation}
with $\omega_{\mu\mu^{\prime}}=E_{A\mu}-E_{P\mu^{\prime}}$ and the reverse processes given by the Hermitian conjugates at $-\omega_{\mu\mu'}$.
Explicit expressions for the coefficients $C_{\mu\mu^{\prime}}$ 
are given in the Supplemental Material.
%
Together, Eqs.~(\eqref{eq:cavity_jumps})--(\eqref{eq:photon_qubit_jumps}) 
and the phonon-induced operators fully determine the Lindblad generator. 

\paragraph{First-order polaron correction to the phonon coupling}

If the phonon coupling operator is retained to first order in
$\lambda$, one must also include the term
\begin{equation}
S_\nu^{(1)}
=
2i\lambda(a^\dagger-a)
\big(\alpha_1\sigma_y^{(1)}-\alpha_2\sigma_y^{(2)}\big).
\end{equation}

This term couples qubit and cavity degrees of freedom and therefore
induces phonon-assisted sideband transitions that simultaneously
change the qubit manifold and the cavity occupation
\begin{equation}
\ket{P\mu',n}\longleftrightarrow\ket{\mathrm{AP}\mu,n\pm1}
\end{equation}
with Bohr frequencies $\omega_{\mu\mu'}\pm\omega_c$.
The corresponding eigenoperator components are therefore
\begin{align}
L_\nu^{(1)}(\omega_{\mu\mu'}+\omega_c)
&=\sqrt{\gamma(\omega_{\mu\mu'}+\omega_c)}
\sum_{n\ge0}
\sqrt{n+1}\,\widetilde{C}_{\mu\mu'}\\
& \ket{\mathrm{AP}\mu,n+1}\!\bra{P\mu',n},
\\
\end{align}
with the reverse processes given by the Hermitian conjugates at $-\omega_{\mu\mu'}$ and/or $-\omega_c$.
%
\begin{comment}
The collapse-operator set includes:
\begin{itemize}
\item \textbf{Cavity loss/absorption:} $L_a=\sqrt{\kappa_\downarrow}\,a$ and $L_{a^\dagger}=\sqrt{\kappa_\uparrow}\,a^\dagger$,
with rates determined by the photon bath at $\pm\omega_c$.
\item \textbf{Photon-induced qubit channels (from polaron-frame coupling):} additional effective jumps within the dressed
antiparallel manifold of the two-qubit Hamiltonian, including relaxation/excitation at $\pm \omega_{\mathrm{ap}}$ and a
zero-frequency dephasing channel.
\item \textbf{Phonon-induced channels:} dressed-basis relaxation/excitation and dephasing within both parallel and
antiparallel manifolds, plus cross-manifold transitions (single-qubit flips) depending on the phonon-coupling operator.
\end{itemize}
In the Supplemental Material we provide explicit expressions for these operators in terms of the mixing angles and bath
rates, in a form directly implementable in QuTiP.
\end{comment}

==> main/main_collision.tex <==
% =========================
\section{Collision-model formulation: simultaneous and sequential beam-splitter--Kerr dynamics}
\label{sec:collision_main}
% =========================

The effective Markovian dynamics derived in Sec.~\ref{sec:lindblad_main} admits a repeated-interaction, or collision-model, realization. In this formulation, the dressed qubit-cavity system interacts during each short time step $\Delta t$ with fresh ancillas modeling photon and phonon environmental excitations. Constructed at the level of the effective dressed coupling operators entering the open-system description, this repeated-interaction model reproduces, in the weak-collision continuum limit, the same GKLS generator obtained from the Born--Markov--secular treatment.

The collision-model viewpoint is particularly useful here because it accommodates both of the control scenarios discussed in Sec.~\ref{sec:ideal}: a simultaneous implementation, in which the red-sideband and Kerr terms act during the same interval, and a sequential implementation, in which the beam-splitter and Kerr evolutions are applied in separate time windows. We discuss these two cases in turn.

\subsection{Repeated-interaction construction}

We write the one-step collision map as
\begin{equation}
\rho(t+\Delta t)
=
\Tr_{\rm anc}
\!\left[
U_{\Delta t}
\big(
\rho(t)\otimes \eta
\big)
U_{\Delta t}^\dagger
\right],
\label{eq:coll_map_rewrite}
\end{equation}
where $\eta$ denotes the state of the fresh ancillas and
\begin{equation}
U_{\Delta t}
=
\exp\!\left[
-i\Delta t\,H_{\rm eff}
-i\sqrt{\Delta t}\sum_{r=\gamma,\nu}V_r
\right].
\label{eq:U_coll_rewrite}
\end{equation}
Here $H_{\rm eff}$ is the coherent system Hamiltonian, while $V_\gamma$ and $V_\nu$ describe the collision couplings associated with the photon and phonon sectors. The $\sqrt{\Delta t}$ scaling is the standard weak-collision scaling ensuring a finite dissipative contribution in the continuum limit.

For each bath label $r\in\{\gamma,\nu\}$, we decompose the corresponding effective system coupling operator into eigenoperators of a reference Hamiltonian $H_0$,
\begin{equation}
S_r=\sum_\omega S_r(\omega),
\qquad
[H_0,S_r(\omega)]=-\omega S_r(\omega).
\label{eq:eigenop_collision_rewrite}
\end{equation}
Choosing the collision Hamiltonians in the rotating form
\begin{equation}
V_r=
\sum_{\omega>0}
\Big(
S_r(\omega)\otimes b_{r,\omega}^\dagger
+
S_r^\dagger(\omega)\otimes b_{r,\omega}
\Big)
+
S_r(0)\otimes X_r ,
\label{eq:Vr_rewrite}
\end{equation}
and assuming vanishing ancilla first moments, the expansion of Eq.~\eqref{eq:coll_map_rewrite} to order $\Delta t$ yields
\begin{equation}
\dot\rho
=
-i[H_{\rm eff}+H_{\rm LS},\rho]
+
\sum_{r,\omega>0}
\Gamma_r^\downarrow(\omega)\,
\mathcal D[S_r(\omega)]\rho
+
\sum_{r,\omega>0}
\Gamma_r^\uparrow(\omega)\,
\mathcal D[S_r^\dagger(\omega)]\rho
+
\sum_r
\Gamma_r^0\,
\mathcal D[S_r(0)]\rho,
\label{eq:GKLS_collision_rewrite}
\end{equation}
where the rates are fixed by ancilla second moments. Thus, once the relevant eigenoperators $S_r(\omega)$ are identified, the collision-model continuum limit directly yields the corresponding Lindblad operators.

\subsection{Simultaneous beam-splitter and Kerr evolution}

We first consider the most general effective setting, in which the red-sideband and Kerr terms act during the same interval,
\begin{equation}
H_{\rm eff}^{({\rm sim})}
=
H_{\rm rsb}
+
H_K
+
H_{\rm diag},
\qquad
H_K=\chi (a^\dagger a)^2.
\label{eq:Heff_simul}
\end{equation}
As in Sec.~\ref{sec:lindblad_main}, the cavity-assisted exchange term is retained in the coherent dynamics, while the dissipative eigenoperator decomposition is performed with respect to a reference Hamiltonian. To include Kerr exactly at this level, we take
\begin{equation}
H_0^{(K)}
=
H_{\rm qb}^{\rm dressed}
+
\omega_c N
+
\chi N^2,
\qquad
N=a^\dagger a.
\label{eq:H0K_main}
\end{equation}
This keeps the Kerr-induced number dependence of the cavity spectrum, while still neglecting the finer hybridization induced by the red-sideband coupling in the dissipator construction. The approximation is therefore consistent whenever the bath does not resolve the additional splittings induced by the qubit-cavity hybridization.

For the photon sector, the effective polaron-frame coupling is
\begin{equation}
S_\gamma^P=a+a^\dagger-2\lambda Z,
\qquad
Z=\sigma_z^{(1)}-\sigma_z^{(2)}.
\label{eq:SgammaP_rewrite}
\end{equation}

The Kerr term modifies the cavity contribution by resolving adjacent Fock-state transitions. Writing
\begin{equation}
a=\sum_{n\ge1} a_n,
\qquad
a_n=\sqrt n\,|n-1\rangle\langle n|,
\end{equation}
one finds
\begin{equation}
[H_0^{(K)},a_n]
=
-\omega_n a_n,
\qquad
\omega_n=\omega_c+\chi(2n-1).
\label{eq:an_kerr_freq}
\end{equation}
Thus the cavity-loss and absorption channels become number resolved:
\begin{equation}
\sum_{n\ge1}
\Gamma_\gamma^\downarrow(\omega_n)\,
\mathcal D[a_n]\rho
+
\sum_{n\ge1}
\Gamma_\gamma^\uparrow(\omega_n)\,
\mathcal D[a_n^\dagger]\rho.
\label{eq:kerr_resolved_cavity}
\end{equation}
In the unresolved-Kerr regime, where the bath cannot distinguish the shifted transition frequencies over the occupied manifold, these channels reduce to the coarse-grained dissipator built from the usual collapse operators $a$ and $a^\dagger$.

The qubit part of Eq.~\eqref{eq:SgammaP_rewrite} is instead unaffected by Kerr at the level of Bohr frequencies, because $Z$ does not change the cavity occupation. Projecting onto the dressed antiparallel manifold gives
\begin{align}
S_\gamma(\omega_{\rm ap})
&=
4\lambda\sin(2\theta_{\rm ap})\,
|AP-\rangle\langle AP+|
\otimes
\mathbb I_{\rm cav},
\\
S_\gamma(-\omega_{\rm ap})
&=
4\lambda\sin(2\theta_{\rm ap})\,
|AP+\rangle\langle AP-|
\otimes
\mathbb I_{\rm cav},
\\
S_\gamma(0)
&=
4\lambda\cos(2\theta_{\rm ap})
\Big(
|AP+\rangle\langle AP+|
-
|AP-\rangle\langle AP-|
\Big)
\otimes
\mathbb I_{\rm cav}.
\label{eq:Z_eigenops_sim}
\end{align}
Substituting these operators into Eq.~\eqref{eq:GKLS_collision_rewrite} reproduces the photon-induced dressed-state relaxation, excitation, and dephasing channels already obtained in Sec.~\ref{sec:lindblad_main}, while refining the cavity dissipation into the Kerr-resolved form of Eq.~\eqref{eq:kerr_resolved_cavity}.

Therefore, in the simultaneous picture the main effect of including Kerr in the collision-model derivation is to make the cavity photon jumps number selective, whereas the photon-induced qubit channels generated by the polaron term retain the same structure as in the Kerr-free treatment.

\subsection{Sequential beam-splitter and Kerr implementation}

We now consider the sequential implementation discussed in Sec.~\ref{sec:ideal}, in which the target gate is applied as
\begin{equation}
U_{\rm target}\simeq U_{BS}U_K,
\qquad
U_K=\exp[-it_K\chi(a^\dagger a)^2].
\end{equation}
In this case the collision-model interpretation becomes literally stroboscopic: one alternates short coherent layers generated by the active Hamiltonian of the current step with collision layers representing dissipation during that step.

During the beam-splitter window, the relevant coherent Hamiltonian is the red-sideband Hamiltonian, and the collision-model continuum limit reproduces the same dissipative channels as in Sec.~\ref{sec:lindblad_main}. During the Kerr window, the coherent evolution is generated by
\begin{equation}
H_{\rm eff}^{({\rm Kerr})}
=
H_{\rm qb}^{\rm dressed}
+
\omega_c N
+
\chi N^2,
\end{equation}
so that the photon collision channels reduce to the Kerr-resolved cavity transitions of Eq.~\eqref{eq:kerr_resolved_cavity}. In this step, the qubit sector acts as a spectator unless additional control fields or residual qubit-cavity couplings are retained.

The sequential picture is therefore simpler both conceptually and operationally. It separates the coherent beam-splitter and Kerr updates into distinct layers, while keeping the same ancilla-based realization of the dissipative environment. This makes the collision-model formulation particularly natural for stroboscopic simulation strategies and for automaton-style architectures in which local coherent updates are interleaved with local noise, reset, or dephasing layers.




==> main/main_perspectives.tex <==
% =========================
\section{Quantum Cellular Automata and collision model perspectives}
\label{sec:perspectives_collision}
% =========================

The collision-model reformulation developed in Sec.~\ref{sec:lindblad_main} is useful not only as an alternative derivation of the effective Lindblad equation, but also as a broader conceptual framework for interpreting the role of the hybrid gate in quantum cellular automata, open-system simulation, and dynamical quantum information processing.

\subsection{Lattice gauge simulation via QCA}
A central motivation for the hybrid beam-splitter gate considered here comes from quantum-cellular-automaton (QCA) approaches to lattice gauge simulation, in particular Schwinger-model-inspired constructions \cite{SellapillayArrighiDiMolfettaQCAQED} in which a bosonic degree of freedom mediates local matter-field updates. In that setting, the present gate provides a natural local update rule for a hybrid QCA architecture in which the qubit sector encodes matter-like degrees of freedom and the cavity mode plays the role of a dynamical bosonic field.


The physical realization discussed here preserves the same local exchange structure, while resolving it into invariant photon-number sectors. Each sector undergoes a two-level Rabi rotation with angle $g_{\mathrm{eff}}t_{BS}\sqrt{n+1}$, as detailed in the Supplemental Material. In this sense, the cQED implementation realizes the same local update mechanism in a block-resolved form adapted to the explicit bosonic Hilbert space.
In addition, the appearance of $a$ and $a^\dagger$ is reversed with respect to the target gate used in the QCA setting. \textcolor{red}{This apparent mismatch can be reinterpreted as a choice of link orientation in the underlying Kogut--Susskind picture, as shown in the Supplemental Material. (should the demosntration be put in the supp or in the next paper?)} Residual phase differences with the target unitary on diagonal and antidiagonal terms can, in principle, be compensated by suitable relative phase gates.



Moreover, from the QCA viewpoint, the cavity is not reset after each update, but it must remain part of the active dynamics, since it stores the local bosonic field information entering the gauge-preserving rule. In the same spirit, the Kerr term is not merely an additional nonlinearity, but a mechanism generating the field-dependent phases required by the automaton update. This viewpoint also clarifies the relation with Markovianity. At the level of the full qubit-cavity system considered in Sec.~\ref{sec:lindblad_main}, the effective evolution remains Markovian, with only the external photon and phonon baths traced out. Memory effects arise only after a further reduction of description, namely when the cavity itself is eliminated and one focuses on the reduced matter dynamics. In that reduced picture, the persistence of the cavity state across successive updates acts as a source of memory. In this operational sense, gauge preservation and non-Markovianity become linked in the present architecture: not because they are equivalent notions in general, but because implementing the gauge-preserving update requires a bosonic mediator that retains information from one step to the next.

\subsection{Open-system simulation and stroboscopic architectures}

The collision model picture also provides a natural language for algorithmic and digital-analog simulation strategies. In the Markovian setting developed in Sec.~\ref{sec:lindblad_main}, the effective evolution may be viewed as the composition of short coherent updates generated by the hybrid qubit-boson Hamiltonian and local collision layers generated by refreshed ancillas. This is precisely the structure naturally implemented in repeated-interaction simulation schemes, where unitary system evolution is interleaved with short ancilla-system couplings followed by ancilla discard or reset.

In the present platform, this viewpoint is especially natural because the coherent sector is already organized around a local hybrid primitive, namely the red-sideband beam-splitter gate composed with Kerr evolution. In a sequential implementation, one may therefore regard the dynamics as a stroboscopic alternation of three elementary layers: a coherent beam-splitter step, a Kerr step, and a dissipative collision step. The collision-model derivation shows that, in the weak-collision continuum limit, this layered construction reproduces the same effective Lindblad dynamics as the standard Born--Markov--secular treatment.

From an algorithmic perspective, the hybrid nature of the primitive is also appealing. Because the cavity provides a bosonic register while the dressed qubit manifold supplies a controllable two-level subsystem, the same architecture supports local matter-field exchange, number-dependent phase accumulation, and engineered dissipation within a single module. This combination is well suited to digital-analog strategies in which nontrivial local terms are implemented natively while the global dynamics is assembled stroboscopically. In particular, the collision-model formulation provides a natural language for distributing dissipation locally across such updates, rather than treating decoherence solely as an uncontrolled external perturbation.

More broadly, the repeated-interaction framework clarifies how the same architecture may interpolate between different simulation regimes. With refreshed ancillas, one obtains a controlled Markovian simulator of the effective Lindblad dynamics. With partial ancilla reuse, correlated ancilla streams, or persistent mediating modes, one is naturally led to controlled departures from the Markovian regime. Hybrid qubit-boson architectures of the present type may therefore provide useful testbeds not only for open-system simulation, but also for the transition between memoryless and memory-bearing quantum dynamics in locally updated many-body settings.

\subsection{From collision models and noisy QCA to quantum reservoir computing}

A further perspective concerns the use of noisy, locally updated quantum dynamics as a computational resource. Quantum reservoir computing (QRC) is attractive from a quantum-machine-learning perspective because it uses a fixed dynamical system as a high-dimensional nonlinear reservoir and trains only a classical readout layer, making it especially well suited to noisy or analog near-term hardware \cite{GhoshQRP,AraizaBravoQRC,SanniaDissipativeQRC}. In this setting, dissipation is not necessarily a detrimental effect: it can instead provide the fading-memory mechanism that makes temporal information processing possible \cite{SanniaDissipativeQRC}.

From this viewpoint, collision models supply a natural microscopic language for reservoir-type processing. Repeated interactions provide a built-in mechanism for sequential input injection, controlled forgetting, and tunable memory through the choice between refreshed and correlated ancillas. Noisy QCA \cite{AvalleSerafiniNoisyQCA} suggest a natural intermediate architectural layer between collision models and reservoir computing: collision models specify local dissipative update mechanisms, while noisy QCA organize such updates into a spatially distributed dynamical medium that propagates and mixes information across space and time. From this viewpoint, reservoir-style processing may be understood as a possible computational use of precisely this kind of noisy, memory-bearing dynamics.

This perspective is supported indirectly by recent progress in quantum reservoir computing. On the one hand, dissipative and reset-based reservoir architectures have been shown to use open-system effects as computational resources rather than mere imperfections \cite{SanniaDissipativeQRC}. On the other hand, QRC is increasingly being explored on realistic tasks and hardware platforms, including realized-volatility forecasting \cite{LiQRCFinance} and credit-default prediction on neutral-atom hardware \cite{VitaliQRCCredit}. Although these works are not formulated in the explicit language of collision models, they reinforce the idea that structured noisy dynamics can be computationally useful in physically relevant settings.

In the present platform, this suggests two natural directions. First, a simplified transversally coupled version of the architecture could realize a cavity-mediated driven-dissipative spin reservoir closely analogous to existing continuous-dissipation spin-network proposals. Second, the full hybrid qubit-boson architecture studied here points to a richer class of reservoir in which a persistent bosonic mode, beam-splitter exchange, engineered dissipation, and optional Kerr nonlinearity are all available within a single module. From this viewpoint, the same features that motivate the gate for QCA and open-system simulation also make it a promising candidate primitive for reservoir-style quantum information processing. Exploring these directions quantitatively, for instance through the benchmark metrics commonly used in the QRC literature, is a natural continuation of the present work.
\section{Conclusion}

In this work, we have introduced a hybrid qubit-boson beam-splitter gate acting between a dressed two-level qubit manifold and a microwave cavity mode in the presence of Kerr nonlinearity. Starting from a general effective model, with carbon-nanotube circuit QED as a concrete implementation, we derived the corresponding effective qubit-cavity exchange interaction and discussed its composition with Kerr evolution in both simultaneous and sequential control regimes.

We then developed an open-system description including photon- and phonon-induced dissipation. The same effective master equation was obtained in two complementary ways, from a standard Born--Markov--secular treatment and from a repeated-interaction collision-model construction. In the weak-dissipation regime, this allowed us to derive a compact analytical expression for the average gate fidelity and to benchmark it against numerical simulations.

Taken together, these results identify the hybrid gate as a useful primitive for engineered qubit-boson dynamics in noisy settings. Beyond the specific circuit-QED realization considered here, the same framework opens natural directions toward quantum cellular automata, lattice-gauge-inspired architectures, ancilla-based open-system simulation, and reservoir-style quantum information processing, e.g. quantum machine learning, based on structured dissipation and memory.

\textcolor{red}{comments on experimental part}

